ChatGPT is a Potential Zero-Shot Dependency Parser

Pre-trained language models have been widely used in dependency parsing task and have achieved significant improvements in parser performance. However, it remains an understudied question whether pre-trained language models can spontaneously exhibit the ability of dependency parsing without introducing additional parser structure in the zero-shot scenario. In this paper, we propose to explore the dependency parsing ability of large language models such as ChatGPT and conduct linguistic analysis. The experimental results demonstrate that ChatGPT is a potential zero-shot dependency parser, and the linguistic analysis also shows some unique preferences in parsing outputs.

==> section/c.introduction.tex <==
\section{Introduction}
Dependency Parsing is a fundamental task in Natural Language Processing.
Previous research of dependency parsing reach the grain performance in paradigm of supervised and semi-supervised dependency parsing\cite{?}.
However, the zero-shot dependency parsing has always been a difficult problem due to the complexity of the parsing task.

Large Language Models such as ChatGPT\cite{?} and GPT-4\cite{?} are the revolutionary progress in Natural Language Processing.
With the help of LLMs’ powerful capabilities and good generalization, we are delighted to find that we can finally achieve zero-shot dependency parsing.
However, the performance of the zero-shot dependency parsing is still not satisfactory.


It is 
In this paper, we analyze in detail the errors that LLMs make in the annotation of dependency parsing from the perspective of linguistics, summarize x kinds of error preferences, and further explore how to use prompt interaction to correct these errorsv  
In addition, we also used Probing to obtain the results of dependency parsing from the previous PLM, and also performed linguistic analysis on these results

